Arbitrary Video Style Transfer via Multi-Channel Correlation

Video style transfer is getting more attention in AI community for its numerous applications such as augmented reality and animation productions. Compared with traditional image style transfer, performing this task on video presents new challenges: how to effectively generate satisfactory stylized results for any specified style, and maintain temporal coherence across frames at the same time. Towards this end, we propose Multi-Channel Correction network (MCCNet), which can be trained to fuse the exemplar style features and input content features for efficient style transfer while naturally maintaining the coherence of input videos. Specifically, MCCNet works directly on the feature space of style and content domain where it learns to rearrange and fuse style features based on their similarity with content features. The outputs generated by MCC are features containing the desired style patterns which can further be decoded into images with vivid style textures. Moreover, MCCNet is also designed to explicitly align the features to input which ensures the output maintains the content structures as well as the temporal continuity. To further improve the performance of MCCNet under complex light conditions, we also introduce the illumination loss during training. Qualitative and quantitative evaluations demonstrate that MCCNet performs well in both arbitrary video and image style transfer tasks.

==> figs/fig_correlation.tex <==
\begin{figure}[!h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/correlation.pdf}
\caption{Comparison with MAST and SANet. The second row is heat maps that used to visualize the differences between two adjacent video frames.}
\label{fig:correction}
\end{figure}


==> figs/fig_sup1.tex <==
\begin{figure*}%[!h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/sup.pdf}
\caption{Comparison of artistic style transfer results. The first column shows style images, the second column shows content images. The remaining columns are stylized results of different methods.
%our methods, MAST~\citep{deng:2020:arbitrary},
% DFP~\citep{wang:2020:diversified}
% Linear~\citep{li:2019:learning}, SANet~\citep{park:2019:arbitrary}, AAMS~\citep{yao:2019:attention}, WCT~\citep{li:2017:universal}, AdaIN~\citep{Huang:2017:Arbitrary}, and NST~\citep{gatys:2016:image}.
}
\label{fig:sup1}
\end{figure*}

==> figs/fig_video_frame.tex <==
\begin{figure*}
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/video_frames.pdf}
\caption{Our video style transfer results. }
\label{fig:frame}
\end{figure*}

==> figs/fig_weight.tex <==
\begin{figure}%[!h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/weight.pdf}
\caption{Influence of style weight.}
\label{fig:weight}
\end{figure}

==> tables/tab_efficiency.tex <==
\begin{table}[t]
\centering

\begin{tabular}{cccccc}
\toprule
Image size&256& 512& 1024 \\
\midrule
Ours&0.013& 0.015& 0.019 \\

MAST&0.030&0.096& 0.506 \\

CompoundVST&0.049&0.098&0.285 \\

DFP&0.563&0.724& 1.260 \\

Linear&0.010&0.013& 0.022 \\

SANet&0.015& 0.019& 0.021 \\

AAMS&2.074& 2.173& 2.456 \\

AdaIN&0.007&0.008& 0.009 \\

WCT&0.451& 0.579& 1.008 \\
 
NST&19.528& 37.211& 106.372 \\
\bottomrule
\end{tabular}
\caption{Inference time of different methods.}
\label{tab:speed}
\end{table}

